Beyond the Trade-off: Self-Supervised Reinforcement Learning for Reasoning Models' Instruction Following

Reasoning models excel in complex problem solving but exhibit a concerning trade off between reasoning capabilities and instruction following abilities. Existing approaches for improving instruction following rely on stronger external models, creating methodological bottlenecks and practical limitations including increased costs and accessibility constraints. We propose a self-supervised RL framework that leverages reasoning models' own internal signals to improve instruction following capabilities without external supervision. Extensive experiments demonstrate that our framework significantly improves instruction following capabilities while maintaining reasoning performance, offering a scalable and cost-effective approach to enhance instruction following in reasoning models. The data and code are publicly available at https://github.com/Rainier-rq/verl-if.

==> tables/soft_follow.tex <==
\begin{table*}[t]

\renewcommand{\arraystretch}{1.3} % 增加行间距到1.5倍
% 在表格环境之前设置全局字体为罗马字体
\renewcommand{\familydefault}{\rmdefault}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}

\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{6}{c}{Hard  Satisfaction Rate}         & \multicolumn{6}{c}{Soft  Satisfaction Rate}                       \\ \cline{2-13} 
\multicolumn{1}{c}{}                       & L1    & L2    & L3    & L4    & L5    & Avg    & L1    & L2    & L3    & L4    & L5    & Avg    \\ \midrule

DeepSeek-R1-Distill-Qwen-1.5B & 70.5& 58.4&50.6&51.7&39.0&54.0 & 70.5& 67.5 & 66.1 & 64.1 & 61.2 & 65.9 \\
DeepSeek-R1-Distill-Qwen-1.5B-IF & 70.3 & 65.4 & 55.8 & 47.4 & 41.5 & 56.1 & 70.3 & 71.3 & 67.1 & 64.1 & 63.9 & 67.3 \\

DeepSeek-R1-Distill-Qwen-7B & 81.9 & 60.5 & 60.7 & 55.4 & 52.0 & 62.1 & 81.9 & 66.4 & 69.5 & 68.7 & 69.3 & 71.2 \\
DeepSeek-R1-Distill-Qwen-7B-IF & 81.2 & 67.5 & 64.9 & 56.3 & 49.9 & 64.0 & 81.2 & 73.3 & 73.3 & 70.3 & 69.3 & 73.5 \\


DeepSeek-R1-Distill-Qwen-32B & \underline{89.6}&	\underline{78.5}&	\textbf{79.6}&	\underline{70.3}&	\underline{63.7}&	\underline{76.3} & \underline{89.6} & \underline{85.0} & \underline{82.0} & \textbf{82.0} &  \underline{75.1} & \underline{82.7} \\
DeepSeek-R1-Distill-Qwen-32B-IF & \textbf{91.2} & \textbf{82.6} & \underline{78.6} & \textbf{72.2}& \textbf{69.0} & \textbf{78.7} & \textbf{91.2} & \textbf{85.1} & \textbf{84.1} & \underline{79.5} & \textbf{80.4} & \textbf{84.1} \\
\bottomrule

\end{tabular}
}
\caption{
The overall performance on the soft constraint subset of FollowBench. We use
\textbf{bold} for the best results and \underline{underlined} for the second-best results.
}
\label{tab:main_soft}
\end{table*}
